Benchmarking Visual Localization for Autonomous Navigation

This work introduces a simulator-based benchmark for visual localization in the autonomous navigation context. The dynamic benchmark enables investigation of how variables such as the time of day, weather, and camera perspective affect the navigation performance of autonomous agents that utilize visual localization for closed-loop control. The experimental part of the paper studies the effects of four such variables by evaluating state-of-the-art visual localization methods as part of the motion planning module of an autonomous navigation stack. The results show major variation in the suitability of the different methods for vision-based navigation. To the authors' best knowledge, the proposed benchmark is the first to study modern visual localization methods as part of a complete navigation stack. We make the benchmark available at https://github.com/lasuomela/carla_vloc_benchmark.

==> source/tables/accuracies_and_failure_viz.tex <==
\newcommand\mcat{.25 / .50 / 5.0}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}

\hfill%
\begin{minipage}[t]{0.21\linewidth} %0.195
\centering

 %\begin{adjustbox}{width=\linewidth, valign=T}
   \includegraphics[width=1.0\linewidth, trim={16cm 3cm 13cm 2cm},clip]{source/figures/netvlad_r2d2_k5_annotated.png}
   %  trim={13cm 2cm 16cm 3cm}
  % \end{adjustbox}
   
   %  \begin{adjustbox}{width=\linewidth, valign=T}
   \includegraphics[width=1.0\linewidth, trim={16cm 3cm 13cm 2cm},clip]{source/figures/netvlad_r2d2_k8_annotated.png}
   %\end{adjustbox}
   %\captionof{figure}{Crash sites (red marks) of Town01 with NetVLAD+R2D2 and $k=5$ (top) and $k=8$ (bottom).}
   %\captionof{figure}{NetVLAD+ R2D2 crashes $@~k=5$ (top) and $k=8$.}
   \captionof{figure}{NetVLAD + R2D2 crashes, Town01.} \label{fig:crash_sites}
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.76\linewidth}
%\tiny % Using resizebox
%\captionof{table}{The visual localization recall rates for the reference paths. The accuracy thresholds used are T1 ($\le$ 0.25m, $\le$2$^\circ$), T2 ($\le$0.50m,$\le$5$^\circ$) and T3 ($\le$5.00m, $\le$10$^\circ$). Full table for all illumination levels $k$ in the supplementary material.}%
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l l r r r r r r r}
      % \multicolumn{10}{c}{Town01} \\
    %\midrule
    & \multirow{2}{*}{PR} & \multirow{2}{*}{LF} & $k=$ 0 & 2 & 4 & 6 & 8 & 10  \\
    %\midrule
    %& &  & \mcat\  & \mcat\  & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\   \\
    %& &  & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\   \\
    &  &   & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 \\
    %\midrule
    \cmidrule(lr){2-9}
   \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=r]{90}{Town01}}}
       
   &  Ap- & Sift   & 98.0 / 98.2 / 99.8 & 84.7 / 89.6 / 96.5 & 85.9 / 89.3 / 96.7 & 73.8 / 78.5 / 90.5 & 19.2 / 23.8 / 29.8 & 3.5 / 5.8 / 8.6     \\
    
    & GeM & D2-net   & 92.3 / 95.7 / 99.8 & 67.3 / 74.7 / 90.1 & 69.1 / 74.7 / 88.0 & 46.9 / 58.1 / 73.8 & 8.6 / 10.9 / 15.6 & 0.5 / 0.8 / 2.0   \\
     
   &  & R2D2   & 98.0 / 98.4 / \textbf{100.0} & 85.5 / 90.4 / 97.7 & 80.6 / 88.2 / 97.0 & 73.3 / 79.7 / 93.6 & 31.7 / 37.5 / 50.5 & 11.2 / 12.9 / 15.0    \\
     
   &  & SuperPoint  & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{99.8} / \textbf{99.8} / 99.8 & 99.5 / \textbf{100.0} / \textbf{100.0} & \textbf{95.9} / 98.5 / 99.0 & 81.7 / 86.3 / 90.5 & 43.7 / 48.9 / 57.9   \\
    \cmidrule(lr){2-9}
    
  
  & Net- & Sift   & 97.4 / 98.5 / 99.8 & 84.4 / 87.7 / 97.5 & 87.2 / 89.8 / 97.4 & 73.2 / 79.6 / 92.3 & 21.9 / 27.0 / 34.4 & 5.8 / 8.2 / 13.0      \\
    
    & VLAD & D2-net   & 96.1 / 96.9 / 99.7 & 69.9 / 75.8 / 90.1 & 67.9 / 75.7 / 87.3 & 43.8 / 52.4 / 75.0 & 10.0 / 13.0 / 17.9 & 0.5 / 1.2 / 1.8      \\
     
    & & R2D2   & 98.4 / 98.5 / 99.7 & 86.5 / 91.0 / 97.5 & 86.2 / 89.5 / 97.5 & 76.6 / 82.4 / 93.1 & 31.6 / 37.7 / 49.2 & 13.8 / 15.3 / 18.3      \\
     
    & & SuperPoint   & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & 99.7 / 99.7 / \textbf{100.0} & \textbf{99.8} / \textbf{100.0} / \textbf{100.0} & 94.4 / \textbf{99.2} / \textbf{99.5} & \textbf{86.2} / \textbf{90.8} / \textbf{96.1} & \textbf{56.4} / \textbf{60.4} / \textbf{68.1}  \\
     
     \cmidrule(lr){2-9} \\
      %\cmidrule(lr){2-11}
     %\\
    %\multicolumn{10}{c}{Town10} \\
    %\midrule
    \cmidrule(lr){2-9}
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=r]{90}{Town10}}}
       & Ap- & Sift  &   
         95.2 / 96.4 / 99.6 & 89.5 / 90.3 / 92.7 & 87.1 / 87.9 / 91.5 & 76.6 / 79.0 / 83.9 & 12.5 / 16.5 / 33.5 & 0.0 / 0.4 / 3.6
        \\
    
   & GeM & D2-net   &  
    94.7 / 98.4 / 99.2 & 84.2 / 88.7 / 91.9 & 81.9 / 87.1 / 92.7 & 46.8 / 53.6 / 65.3 & 0.0 / 0.0 / 1.2 & 0.0 / 0.0 / 0.0
     \\
     
    & & R2D2   & 
     93.1 / 94.7 / 99.6 & 88.3 / 90.7 / 92.3 & 85.5 / 87.9 / 90.3 & 75.8 / 78.2 / 83.5 & 15.7 / 21.4 / 31.5 & 0.4 / 0.8 / 2.8
     \\
     
   &  & SuperPoint   &   
    99.6 / \textbf{100.0} / \textbf{100.0} & 96.0 / 96.0 / 96.0 & 94.4 / 94.4 / 94.4 & 93.1 / 93.5 / 93.5 & 73.4 / 75.4 / 76.2 & 35.9 / 37.5 / 41.5
     \\
    %\midrule
    \cmidrule(lr){2-9}
    
   & Net- & Sift   &   
    96.4 / 97.2 / \textbf{100.0} & 92.7 / 94.0 / 94.8 & 87.9 / 90.7 / 93.5 & 75.4 / 77.8 / 85.1 & 12.9 / 17.3 / 35.5 & 0.4 / 0.4 / 2.0
    \\
    
    & VLAD & D2-net   &   
      97.2 / 99.6 / \textbf{100.0} & 86.7 / 89.5 / 94.0 & 83.1 / 88.3 / 92.7 & 45.2 / 58.5 / 69.4 & 0.0 / 0.0 / 0.8 & 0.0 / 0.0 / 0.0
     \\
     
   &  & R2D2  &   
     91.6 / 92.8 / 99.6 & 88.7 / 91.1 / 92.7 & 85.9 / 89.1 / 90.7 & 76.6 / 80.6 / 87.1 & 14.1 / 20.2 / 33.9 & 0.4 / 0.8 / 2.0
     \\
     
   &  & SuperPoint   &  
       \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{97.2} / \textbf{97.2} / \textbf{97.6} & \textbf{97.6} / \textbf{98.0} / \textbf{98.0} & \textbf{98.0} / \textbf{98.0} / \textbf{98.0} & \textbf{86.7} / \textbf{87.9} / \textbf{88.7} & \textbf{50.0} / \textbf{55.2} / \textbf{58.1}
     \\
     
     %\bottomrule
     \cmidrule(lr){2-9}
          \cmidrule(lr){2-9}
  \end{tabular}
}
\captionof{table}{The localization recall rates for the reference paths with thresholds T1 ($\le$ 0.25m, $\le$2$^\circ$), T2 ($\le$0.50m,$\le$5$^\circ$) and T3 ($\le$5.00m, $\le$10$^\circ$). Table with all values of $k$ in the appendix.}\label{tab:accuracies}
\end{minipage}%
%\hfill

==> source/tables/accuracies_full.tex <==

% ECCV RESULTS!!

\newcommand\mcat{.25 / .50 / 5.0}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}
%\tiny % Using resizebox
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l l r r r r r r r}
      % \multicolumn{10}{c}{Town01} \\
    %\midrule
    &  &  & $k=$ 0 & 2 & 4 & 6 & 8 & 10  \\
    %\midrule
    %& &  & \mcat\  & \mcat\  & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\   \\
    %& &  & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\   \\
   & &   & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 \\
    %\midrule
    \cmidrule(lr){2-9}
   \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=r]{90}{Town01}}}
       
   &  Ap-GeM & Sift   & 96.4 / 97.0 / 98.0 & 83.7 / 87.3 / 94.9 & 82.4 / 85.0 / 92.3 & 69.2 / 73.1 / 85.3 & 19.8 / 23.5 / 30.6 & 3.6 / 4.7 / 8.8     \\
    
    & & D2-net   & 92.6 / 95.6 / 99.5 & 70.5 / 77.2 / 90.8 & 69.7 / 75.8 / 89.3 & 46.9 / 56.4 / 75.7 & 9.3 / 12.3 / 16.4 & 0.8 / 1.3 / 2.3   \\
     
   &  & R2D2   & 95.2 / 97.2 / 99.0 & 82.7 / 88.7 / 96.2 & 81.6 / 86.0 / 97.0 & 72.2 / 79.4 / 92.0 & 27.6 / 34.0 / 44.7 & 9.2 / 12.2 / 14.0    \\
     
   &  & SuperPoint  & 99.2 / 99.2 / 99.2 & 97.0 / 98.0 / 98.0 & 96.9 / 97.9 / 97.9 & 93.6 / 94.7 / 94.9 & 67.3 / 72.5 / 77.6 & 35.5 / 38.8 / 47.0   \\
    \cmidrule(lr){2-9}
    
  
  & NetVLAD & Sift   & 95.7 / 97.2 / 99.0 & 87.0 / 91.3 / 98.0 & 85.9 / 90.0 / 96.2 & 71.6 / 79.0 / 90.6 & 22.1 / 25.7 / 34.5 & 4.9 / 7.2 / 12.0      \\
    
    & & D2-net   & 94.1 / 95.9 / \textbf{99.8} & 68.8 / 77.0 / 91.2 & 69.7 / 76.3 / 89.3 & 48.7 / 57.1 / 77.6 & 9.6 / 12.3 / 16.2 & 0.5 / 0.8 / 2.6      \\
     
    & & R2D2   & 94.4 / 96.9 / \textbf{99.8} & 81.0 / 87.4 / 97.4 & 80.5 / 86.0 / 96.6 & 74.1 / 81.0 / 93.8 & 33.1 / 37.2 / 49.9 & 12.3 / 14.3 / 16.8      \\
     
    & & SuperPoint   & \textbf{99.8} / \textbf{99.8} / \textbf{99.8} & \textbf{98.8} / \textbf{99.3} / \textbf{99.7} & \textbf{98.5} / \textbf{99.2} / \textbf{99.5} & \textbf{97.5} / \textbf{98.2} / \textbf{98.4} & \textbf{69.8} / \textbf{75.1} / \textbf{79.7} & \textbf{39.7} / \textbf{44.3} / \textbf{51.1}  \\
     
     \cmidrule(lr){2-9} \\
      %\cmidrule(lr){2-11}
     %\\
    %\multicolumn{10}{c}{Town10} \\
    %\midrule
    \cmidrule(lr){2-9}
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=r]{90}{Town10}}}
       & Ap-GeM & Sift  &   
         94.4 / 98.4 / 99.6 & 89.6 / 91.2 / 92.8 & 90.1 / 91.3 / 93.3 & 72.8 / 76.8 / 81.5 & 11.2 / 15.7 / 30.9 & 0.0 / 1.6 / 4.0
        \\
    
   &  & D2-net   &  
    98.0 / 99.6 / \textbf{100.0} & 87.2 / 90.4 / 93.2 & 82.1 / 86.5 / 92.1 & 47.6 / 58.8 / 66.4 & 0.0 / 0.0 / 0.8 & 0.0 / 0.0 / 0.0  
     \\
     
    & & R2D2   & 
    87.3 / 90.4 / 99.6 & 90.5 / 92.1 / 92.9 & 84.0 / 85.6 / 91.6 & 74.6 / 76.6 / 83.3 & 13.2 / 18.0 / 27.6 & 0.0 / 0.8 / 1.6  
     \\
     
   &  & SuperPoint   &   
    98.4 / 98.8 / 99.2 & 95.6 / 96.4 / 96.4 & 96.0 / 96.0 / 96.8 & 92.8 / 93.2 / 93.2 & 64.7 / 66.3 / 67.1 & 30.6 / 33.7 / 36.5  
     \\
    %\midrule
    \cmidrule(lr){2-9}
    
   & NetVLAD & Sift   &   
    94.9 / 97.2 / 98.8 & 94.4 / 94.8 / 96.0 & 88.8 / 90.8 / 92.4 & 79.1 / 84.7 / 88.0 & 13.6 / 19.2 / 36.0 & 0.4 / 0.4 / 2.4  
    \\
    
    & & D2-net   &   
    97.2 / 99.2 / \textbf{100.} & 87.3 / 90.8 / 94.4 & 84.4 / 89.2 / 93.6 & 44.8 / 54.4 / 67.1 & 0.0 / 0.0 / 0.8 & 0.0 / 0.0 / 0.4  
     \\
     
   &  & R2D2  &   
    90.4 / 93.6 / 99.2 & 88.8 / 90.0 / 94.4 & 86.9 / 89.2 / 93.2 & 78.5 / 81.7 / 88.0 & 13.5 / 18.7 / 30.6 & 0.4 / 1.2 / 2.8  
     \\
     
   &  & SuperPoint   &  
     \textbf{99.6} / \textbf{100.} / \textbf{100.} & \textbf{98.0} / \textbf{98.0} / \textbf{98.4} & \textbf{97.6} / \textbf{97.6} / \textbf{98.0} & \textbf{96.8} / \textbf{97.6} / \textbf{97.6} & \textbf{70.3} / \textbf{71.9} / \textbf{73.1} & \textbf{40.9} / \textbf{42.1} / \textbf{45.2}  
     \\
     
     %\bottomrule
     \cmidrule(lr){2-9}
          \cmidrule(lr){2-9}
  \end{tabular}
}
%{c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen}}

==> source/tables/accuracies_short.tex <==


\newcommand\mcat{.25 / .50 / 5.0}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}
%\tiny % Using resizebox
  \centering
  \resizebox{0.8\linewidth}{!}{
  \begin{tabular}{l l r r r r r r r}
      % \multicolumn{10}{c}{Town01} \\
    %\midrule
    &  &  & $k=$ 0 & 2 & 4 & 6 & 8 & 10  \\
    %\midrule
    %& &  & \mcat\  & \mcat\  & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\   \\
    %& &  & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\   \\
   & &   & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 & T1 / T2 / T3 \\
    %\midrule
    \cmidrule(lr){2-9}
   \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=r]{90}{Town01}}}
       
   &  Ap- & Sift   & 98.0 / 98.2 / 99.8 & 84.7 / 89.6 / 96.5 & 85.9 / 89.3 / 96.7 & 73.8 / 78.5 / 90.5 & 19.2 / 23.8 / 29.8 & 3.5 / 5.8 / 8.6     \\
    
    & GeM & D2-net   & 92.3 / 95.7 / 99.8 & 67.3 / 74.7 / 90.1 & 69.1 / 74.7 / 88.0 & 46.9 / 58.1 / 73.8 & 8.6 / 10.9 / 15.6 & 0.5 / 0.8 / 2.0   \\
     
   &  & R2D2   & 98.0 / 98.4 / \textbf{100.0} & 85.5 / 90.4 / 97.7 & 80.6 / 88.2 / 97.0 & 73.3 / 79.7 / 93.6 & 31.7 / 37.5 / 50.5 & 11.2 / 12.9 / 15.0    \\
     
   &  & SuperPoint  & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{99.8} / \textbf{99.8} / 99.8 & 99.5 / \textbf{100.0} / \textbf{100.0} & \textbf{95.9} / 98.5 / 99.0 & 81.7 / 86.3 / 90.5 & 43.7 / 48.9 / 57.9   \\
    \cmidrule(lr){2-9}
    
  
  & Net- & Sift   & 97.4 / 98.5 / 99.8 & 84.4 / 87.7 / 97.5 & 87.2 / 89.8 / 97.4 & 73.2 / 79.6 / 92.3 & 21.9 / 27.0 / 34.4 & 5.8 / 8.2 / 13.0      \\
    
    & VLAD & D2-net   & 96.1 / 96.9 / 99.7 & 69.9 / 75.8 / 90.1 & 67.9 / 75.7 / 87.3 & 43.8 / 52.4 / 75.0 & 10.0 / 13.0 / 17.9 & 0.5 / 1.2 / 1.8      \\
     
    & & R2D2   & 98.4 / 98.5 / 99.7 & 86.5 / 91.0 / 97.5 & 86.2 / 89.5 / 97.5 & 76.6 / 82.4 / 93.1 & 31.6 / 37.7 / 49.2 & 13.8 / 15.3 / 18.3      \\
     
    & & SuperPoint   & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & 99.7 / 99.7 / \textbf{100.0} & \textbf{99.8} / \textbf{100.0} / \textbf{100.0} & 94.4 / \textbf{99.2} / \textbf{99.5} & \textbf{86.2} / \textbf{90.8} / \textbf{96.1} & \textbf{56.4} / \textbf{60.4} / \textbf{68.1}  \\
     
     \cmidrule(lr){2-9} \\
      %\cmidrule(lr){2-11}
     %\\
    %\multicolumn{10}{c}{Town10} \\
    %\midrule
    \cmidrule(lr){2-9}
    \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=r]{90}{Town10}}}
       & Ap- & Sift  &   
         95.2 / 96.4 / 99.6 & 89.5 / 90.3 / 92.7 & 87.1 / 87.9 / 91.5 & 76.6 / 79.0 / 83.9 & 12.5 / 16.5 / 33.5 & 0.0 / 0.4 / 3.6
        \\
    
   & GeM & D2-net   &  
    94.7 / 98.4 / 99.2 & 84.2 / 88.7 / 91.9 & 81.9 / 87.1 / 92.7 & 46.8 / 53.6 / 65.3 & 0.0 / 0.0 / 1.2 & 0.0 / 0.0 / 0.0
     \\
     
    & & R2D2   & 
     93.1 / 94.7 / 99.6 & 88.3 / 90.7 / 92.3 & 85.5 / 87.9 / 90.3 & 75.8 / 78.2 / 83.5 & 15.7 / 21.4 / 31.5 & 0.4 / 0.8 / 2.8
     \\
     
   &  & SuperPoint   &   
    99.6 / \textbf{100.0} / \textbf{100.0} & 96.0 / 96.0 / 96.0 & 94.4 / 94.4 / 94.4 & 93.1 / 93.5 / 93.5 & 73.4 / 75.4 / 76.2 & 35.9 / 37.5 / 41.5
     \\
    %\midrule
    \cmidrule(lr){2-9}
    
   & Net- & Sift   &   
    96.4 / 97.2 / \textbf{100.0} & 92.7 / 94.0 / 94.8 & 87.9 / 90.7 / 93.5 & 75.4 / 77.8 / 85.1 & 12.9 / 17.3 / 35.5 & 0.4 / 0.4 / 2.0
    \\
    
    & VLAD & D2-net   &   
      97.2 / 99.6 / \textbf{100.0} & 86.7 / 89.5 / 94.0 & 83.1 / 88.3 / 92.7 & 45.2 / 58.5 / 69.4 & 0.0 / 0.0 / 0.8 & 0.0 / 0.0 / 0.0
     \\
     
   &  & R2D2  &   
     91.6 / 92.8 / 99.6 & 88.7 / 91.1 / 92.7 & 85.9 / 89.1 / 90.7 & 76.6 / 80.6 / 87.1 & 14.1 / 20.2 / 33.9 & 0.4 / 0.8 / 2.0
     \\
     
   &  & SuperPoint   &  
       \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{97.2} / \textbf{97.2} / \textbf{97.6} & \textbf{97.6} / \textbf{98.0} / \textbf{98.0} & \textbf{98.0} / \textbf{98.0} / \textbf{98.0} & \textbf{86.7} / \textbf{87.9} / \textbf{88.7} & \textbf{50.0} / \textbf{55.2} / \textbf{58.1}
     \\
     
     %\bottomrule
     \cmidrule(lr){2-9}
          \cmidrule(lr){2-9}
  \end{tabular}
}
%{c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen} c@{\hskip \skiplen}}

==> source/tables/streetlight_results.tex <==
\centering
  \resizebox{0.6\linewidth}{!}{
  \begin{tabular}{ c r r }
    & Town01 &  Town10 \\

    \midrule
     Success rate & 
     50.0 & 100.0 \\
     
    T1 / T2 / T3 & 
    54.3 / 70.2 / 96.9 &
    92.6 / 92.9 / 93.1 \\
     \bottomrule
  \end{tabular}
  }


==> source/tables/town01_accuracies_full.tex <==
%\newcommand\mcat{.25 / .50 / 5.0}
\newcommand\mcat{T1 / T2 / T3}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}
%\tiny
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{c c  c c c c c c c c c c c c c c c c c}
  & & \multicolumn{11}{c}{Town01}   \\
    \cmidrule{3-13}
    \vspace{-0.45cm}
    \\
    \cmidrule{3-13}
     \multirow{2}{*}{PR} & \multirow{2}{*}{LF} &  $k=$ 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    \cmidrule{3-13}
    & &   \mcat\  & \mcat\  & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\  \\
    %& &   \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\  \\
    \midrule
    Ap- & Sift  & 98.0 / 98.2 / 99.8 & 89.5 / 92.9 / 99.0 & 84.7 / 89.6 / 96.5 & 86.7 / 89.3 / 96.1 & 85.9 / 89.3 / 96.7 & 85.4 / 89.5 / 95.4 & 73.8 / 78.5 / 90.5 & 45.3 / 51.6 / 63.9 & 19.2 / 23.8 / 29.8 & 9.2 / 11.8 / 16.4 & 3.5 / 5.8 / 8.6  \\
    
     GeM & D2-net   & 92.3 / 95.7 / 99.8 & 79.8 / 86.7 / 97.5 & 67.3 / 74.7 / 90.1 & 68.8 / 74.8 / 90.1 & 69.1 / 74.7 / 88.0 & 62.8 / 70.9 / 85.7 & 46.9 / 58.1 / 73.8 & 24.0 / 28.5 / 39.3 & 8.6 / 10.9 / 15.6 & 2.1 / 3.1 / 6.2 & 0.5 / 0.8 / 2.0  \\
     
     & R2D2   & 98.0 / 98.4 / \textbf{100.0} & 91.9 / 94.1 / 98.7 & 85.5 / 90.4 / 97.7 & 85.7 / 90.6 / 96.2 & 80.6 / 88.2 / 97.0 & 84.5 / 88.0 / 96.5 & 73.3 / 79.7 / 93.6 & 53.0 / 62.8 / 79.1 & 31.7 / 37.5 / 50.5 & 16.6 / 20.4 / 23.6 & 11.2 / 12.9 / 15.0 \\
     
     & SuperPoint  &  \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{99.8} / \textbf{99.8} / 99.8 & 97.7 / 99.8 / \textbf{100.0} & 99.5 / \textbf{100.0} / \textbf{100.0} & 99.2 / 99.3 / 99.7 & \textbf{95.9} / 98.5 / 99.0 & 91.4 / 94.6 / 96.5 & 81.7 / 86.3 / 90.5 & 59.2 / 65.0 / 71.5 & 43.7 / 48.9 / 57.9 \\
   \midrule
    Net- & Sift   & 97.4 / 98.5 / 99.8 & 91.0 / 93.3 / 99.2 & 84.4 / 87.7 / 97.5 & 86.3 / 89.5 / 96.9 & 87.2 / 89.8 / 97.4 & 82.7 / 87.5 / 96.5 & 73.2 / 79.6 / 92.3 & 47.2 / 53.1 / 67.6 & 21.9 / 27.0 / 34.4 & 9.2 / 13.8 / 20.5 & 5.8 / 8.2 / 13.0   \\
    
     VLAD & D2-net   & 96.1 / 96.9 / 99.7 & 77.2 / 85.1 / 98.7 & 69.9 / 75.8 / 90.1 & 68.4 / 74.8 / 90.0 & 67.9 / 75.7 / 87.3 & 65.5 / 71.9 / 86.3 & 43.8 / 52.4 / 75.0 & 24.2 / 29.9 / 42.6 & 10.0 / 13.0 / 17.9 & 2.1 / 4.4 / 8.0 & 0.5 / 1.2 / 1.8   \\
     
     & R2D2   &  98.4 / 98.5 / 99.7 & 84.3 / 91.8 / 98.7 & 86.5 / 91.0 / 97.5 & 83.7 / 87.0 / 97.2 & 86.2 / 89.5 / 97.5 & 83.5 / 87.3 / 96.2 & 76.6 / 82.4 / 93.1 & 58.2 / 66.1 / 83.1 & 31.6 / 37.7 / 49.2 & 19.2 / 22.2 / 27.6 & 13.8 / 15.3 / 18.3  \\
     
     & SuperPoint   &  \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & 99.7 / 99.8 / \textbf{100.0} & 99.7 / 99.7 / \textbf{100.0} & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{99.8} / \textbf{100.0} / \textbf{100.0} & \textbf{99.7} / \textbf{100.0} / \textbf{100.0} & 94.4 / \textbf{99.2} / \textbf{99.5} & \textbf{92.8} / \textbf{96.7} / \textbf{99.7} & \textbf{86.2} / \textbf{90.8} / \textbf{96.1} & \textbf{72.5} / \textbf{78.1} / \textbf{87.2} & \textbf{56.4} / \textbf{60.4} / \textbf{68.1} \\
     
     \bottomrule
     
  \end{tabular}
  }


==> source/tables/town01_accuracies_pitch.tex <==
%\newcommand\mcat{.25 / .50 / 5.0}
\newcommand\mcat{T1 / T2 / T3}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}
%\tiny
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l l r r r r r r r r r r r r r r }
  & & \multicolumn{13}{c}{Town01} &  \\
    \cmidrule{3-15}
    \vspace{-0.45cm}
    \\
    \cmidrule{3-15}
    %\midrule
         % town01
     \multirow{2}{*}{PR} & \multirow{2}{*}{LF} &  $z=$ 0 & 2 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 13 & 15 & 16 &

     \\

      &  &  $\theta=$ 0 & 10 & 22.5 & 27.5 & 32.5 & 35 & 37.5 & 40 & 40 & 40 & 40 & 40 & 40 & \\
    \midrule
    & &   \mcat\  & \mcat\  & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\  \\
    %& &   \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\  \\
    \midrule
    Ap- & Sift  & 98.0 / 98.2 / 99.8 & 95.9 / 96.9 / 97.9 & 87.5 / 89.3 / 93.1 & 78.8 / 83.4 / 88.3 & 66.7 / 72.1 / 78.8 & 58.7 / 65.8 / 74.0 & 50.1 / 57.8 / 65.7 & 38.6 / 47.1 / 55.8 & 36.6 / 41.5 / 49.2 & 29.7 / 38.4 / 46.3 & 21.4 / 26.5 / 33.3 & 17.8 / 21.9 / 31.2 & 17.4 / 22.2 / 29.7  \\
    
     GeM & D2-net   & 92.3 / 95.7 / 99.8 & 89.8 / 95.2 / 98.2 & 26.0 / 46.4 / 76.8 & 10.3 / 21.8 / 53.9 & 4.1 / 9.5 / 23.5 & 1.8 / 8.2 / 21.2 & 1.0 / 3.8 / 13.5 & 0.7 / 2.3 / 8.7 & 0.8 / 1.3 / 8.1 & 0.0 / 0.3 / 5.6 & 0.0 / 0.2 / 2.3 & 0.0 / 0.0 / 1.0 & 0.0 / 0.0 / 0.5  \\
     
     & R2D2   & 98.0 / 98.4 / \textbf{100.0} & 98.0 / 98.0 / 98.5 & 79.6 / 81.4 / 88.8 & 64.1 / 67.6 / 75.5 & 40.3 / 49.7 / 59.9 & 28.5 / 38.5 / 50.2 & 22.2 / 29.9 / 44.1 & 12.7 / 21.2 / 36.0 & 12.2 / 20.2 / 31.7 & 10.5 / 18.3 / 28.6 & 7.4 / 14.8 / 22.9 & 7.6 / 13.0 / 21.1 & 6.1 / 11.5 / 21.1 \\
     
     & SuperPoint  & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & \textbf{99.5} / \textbf{99.5} / \textbf{99.7} & \textbf{96.7} / \textbf{96.7} / \textbf{98.5} & 94.7 / 94.9 / \textbf{97.4} & 89.8 / 90.3 / 94.1 & 85.2 / 86.8 / 92.4 & 81.0 / 83.3 / 88.2 & 74.3 / 76.6 / 83.9 & 69.1 / 72.7 / 80.1 & 65.3 / 70.1 / 76.0 & 54.4 / 60.7 / 66.4 & 45.7 / 52.3 / 57.1 & 42.9 / 49.8 / 54.9  \\
   \midrule
    Net- & Sift   & 97.4 / 98.5 / 99.8 & 96.4 / 96.9 / 97.9 & 88.5 / 90.1 / 93.8 & 81.7 / 85.2 / 89.3 & 69.5 / 75.5 / 82.9 & 61.8 / 67.3 / 73.5 & 55.2 / 61.1 / 68.6 & 45.3 / 52.2 / 63.3 & 39.5 / 46.9 / 55.1 & 38.6 / 44.7 / 52.2 & 26.5 / 33.8 / 43.8 & 23.6 / 27.8 / 36.6 & 20.1 / 23.9 / 30.8   \\
    
     VLAD & D2-net   &  96.1 / 96.9 / 99.7 & 90.3 / 96.7 / 98.7 & 26.3 / 46.6 / 78.5 & 12.3 / 21.2 / 57.2 & 5.6 / 11.3 / 28.2 & 1.5 / 7.4 / 23.0 & 1.2 / 4.8 / 16.8 & 1.5 / 3.0 / 14.1 & 0.3 / 1.3 / 8.9 & 0.3 / 0.8 / 5.9 & 0.0 / 0.0 / 3.3 & 0.0 / 0.0 / 1.3 & 0.0 / 0.0 / 1.6  \\
     
     & R2D2   &  98.4 / 98.5 / 99.7 & 98.4 / 98.4 / 99.0 & 79.3 / 81.1 / 88.7 & 66.2 / 70.8 / 79.3 & 46.6 / 53.5 / 63.4 & 35.7 / 44.1 / 53.3 & 26.3 / 33.3 / 45.5 & 16.1 / 25.6 / 38.6 & 15.9 / 23.0 / 33.4 & 14.1 / 19.0 / 29.2 & 10.2 / 17.2 / 23.8 & 8.2 / 12.6 / 21.2 & 9.0 / 12.8 / 20.2  \\
     
     & SuperPoint   & \textbf{100.0} / \textbf{100.0} / \textbf{100.0} & 99.0 / 99.0 / 99.2 & \textbf{96.7} / \textbf{96.7} / 98.0 & \textbf{95.1} / \textbf{95.1} / \textbf{97.4} & \textbf{91.4} / \textbf{92.3} / \textbf{96.2} & \textbf{87.2} / \textbf{88.3} / \textbf{95.1} & \textbf{81.1} / \textbf{84.9} / \textbf{91.4} & \textbf{77.7} / \textbf{81.1} / \textbf{88.3} & \textbf{72.9} / \textbf{77.0} / \textbf{84.5} & \textbf{68.3} / \textbf{73.8} / \textbf{79.4} & \textbf{60.5} / \textbf{68.3} / \textbf{73.7} & \textbf{54.9} / \textbf{66.1} / \textbf{71.3} & \textbf{53.8} / \textbf{62.0} / \textbf{68.1}  \\
     
     \bottomrule
     
  \end{tabular}
  }


==> source/tables/town01_failures_illumination.tex <==
  \centering
  \resizebox{0.90\linewidth}{!}{
  \begin{tabular}{l l r r r r r r r r r r r r  }
  &  & \multicolumn{11}{c}{Town01}       \\
    \cmidrule(lr){3-13}
    %\midrule
         % town01
     PR & LF &  $k=$ 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 
     \\
    %\midrule
    \midrule
     % town01
    Ap- & Sift  & \textbf{0.0} & 1.8 & 4.8 & 5.5 & 5.1 & 5.1 & 11.6 & 28.3 & 32.1 & 22.8 & 21.4 
    \\
     % town01
     GeM & D2-net  & 0.2 & 7.1 & 11.1 & 12.6 & 12.6 & 13.9 & 20.9 & 26.2 & 21.7 & 14.9 & 20.9
     \\
      % town01
     & R2D2  & 0.2 & 1.5 & 3.8 & 4.3 & 5.0 & 5.1 & 7.8 & 13.4 & 21.4 & 18.0 & 18.7
     \\
     % town01
     & SuperPoint & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.2} & 4.5 & 7.6 & 14.6
     \\
    \midrule
     % town01
    Net- & Sift  & 0.2 & 1.5 & 2.8 & 4.1 & 6.3 & 5.6 & 8.9 & 29.3 & 32.5 & 24.7 & 19.9
    \\
     % town01
     VLAD & D2-net  & 0.3 & 6.8 & 13.2 & 12.7 & 11.9 & 14.6 & 23.0 & 24.8 & 22.2 & 21.2 & 18.0
    \\
    %town01
     & R2D2  & 0.2 & 1.3 & 3.8 & 3.6 & 4.1 & 4.5 & 7.1 & 16.2 & 21.5 & 19.7 & 16.9
     \\
     %town01
     & SuperPoint  & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.2} & \textbf{1.8} & \textbf{5.5} & \textbf{12.3}
     \\
     \midrule
     \multicolumn{2}{l}{Wheel odometry} &  \multicolumn{11}{c}{17.9}
      \\
     \bottomrule
  \end{tabular}
  }

==> source/tables/town01_pitch_k0_failures.tex <==
% VIEWPOINT FAILURES

    \centering 
    \resizebox{0.92\linewidth}{!}{ %0.95
  \begin{tabular}{l l r r r r r r r r r r r r r r }
  & & \multicolumn{13}{c}{Town01} &  \\
    \cmidrule{3-15}
    %\midrule
         % town01
     \multirow{2}{*}{PR} & \multirow{2}{*}{LF} &  $z=$ 0 & 2 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 13 & 15 & 16 &

     \\

      &  &  $\theta=$ 0 & 10 & 22.5 & 27.5 & 32.5 & 35 & 37.5 & 40 & 40 & 40 & 40 & 40 & 40 &

     \\
    %\midrule
    \midrule
     % town01
    Ap- & Sift & \textbf{0.0} & 1.3 & 5.0 & 10.4 & 14.2 & 19.2 & 27.2 & 32.3 & 34.9 & 34.4 & 38.4 & 36.9 & 35.8 & 

    \\
     % town01
     GeM & D2-net  & 0.2 & 2.8 & 29.6 & 42.2 & 38.6 & 31.8 & 34.8 & 29.0 & 31.0 & 29.8 & 29.6 & 25.0 & 23.5 & 
     \\
      % town01
     & R2D2  & 0.2 & 0.7 & 7.0 & 16.2 & 21.0 & 22.5 & 24.7 & 22.8 & 20.5 & 21.2 & 21.0 & 18.7 & 21.2 & 
     \\
     % town01
     & SuperPoint & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.2} & \textbf{1.0} & \textbf{1.8} & 2.2 & \textbf{4.0} & \textbf{5.3} & 7.3 & 9.8 & \textbf{13.7} & 13.1 & 
     \\
     
    \midrule
     % town01
    Net- & Sift  & 0.2 & 1.7 & 4.0 & 9.4 & 14.4 & 19.2 & 26.7 & 30.8 & 34.1 & 35.4 & 37.7 & 39.2 & 41.1 &
    \\
     % town01
     VLAD & D2-net  & 0.3 & 2.8 & 30.1 & 40.7 & 34.6 & 31.5 & 35.3 & 31.6 & 30.5 & 30.8 & 26.3 & 23.0 & 22.4 &
    \\
    %town01
     & R2D2  & 0.2 & 0.7 & 7.8 & 16.6 & 22.0 & 23.0 & 24.0 & 26.0 & 21.2 & 22.0 & 24.0 & 21.7 & 23.2 &
     \\
     %town01
     & SuperPoint  & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & 0.5 & 2.0 & 2.5 & \textbf{1.8} & 4.6 & 6.5 & \textbf{6.6} & \textbf{9.3} & 13.9 & \textbf{12.3} &
     \\
     \midrule
     \multicolumn{2}{l}{Wheel odometry} &  \multicolumn{12}{c}{17.9} %& 17.9 &  &  &  & &  &  &  &  &  &  &  &  
      \\
     \bottomrule
  \end{tabular} %\resizebox{0.33\linewidth}{!}{
  }
  
%  \hfill% 
  %%%%%%%%%%%%%%%%%%%%%%%%
  % BEGIN WEATHER RESULTS
  %%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[t]{0.31\linewidth}
%  \captionof{table}{Failure rates at gallery-to-query weather (visibility) changes $v$.}%
%    \centering
    %\captionof{table}{Blalbla}
%    \resizebox{0.95\linewidth}{!}{ % 1.0
%  \begin{tabular}{l l r r r r }
%   & &\multicolumn{4}{c}{Town01}  \\
%    \cmidrule{3-6}
    %\midrule
         % town01
%    PR & LF & $v=$ 90 & 60 & 30 & 10 

%     \\
    %\midrule
%    \midrule
     % town01
%    Ap- & Sift &  8.5 & 25.4 & 25.4 & 21.9  

%    \\
     % town01
%    GeM & D2-net  & 12.1 & 13.8 & 10.3 & 12.9 
%     \\
      % town01
%     & R2D2  & 10.3 & 12.5 & 10.3 & 10.3 
%     \\
     % town01
%     & SuperPoint & \textbf{0.0} & 0.4 & 1.8 & 2.2 
%     \\
     
 %   \midrule
     % town01
%    Net- & Sift  & 7.6 & 25.9 & 29.5 & 25.9 
%    \\
     % town01
%     VLAD & D2-net  & 12.5 & 13.4 & 10.7 & 9.4
%    \\
    %town01
%     & R2D2  & 9.4 & 8.0 & 7.6 & 8.5  
%     \\
     %town01
%     & SuperPoint  & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.9} 
%     \\
%     \midrule
%     \multicolumn{2}{l}{Wheel odometry}  & \multicolumn{4}{c}{9.8} %& 9.8 &  &  &  
%      \\
%     \bottomrule
%  \end{tabular}
%  }
%  \label{tab:weather_failures}
%  \end{minipage}

==> source/tables/town10_accuracies_full.tex <==
%\newcommand\mcat{.25 / .50 / 5.0}
\newcommand\mcat{T1 / T2 / T3}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}
%\tiny
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{c c  c c c c c c c c c c c c c c c c c}
  &  & \multicolumn{11}{c}{Town10}   \\
    \cmidrule{3-13}
    \vspace{-0.45cm}
    \\
    \cmidrule{3-13}
    \multirow{2}{*}{PR} & \multirow{2}{*}{LF} &  $k=$ 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    \cmidrule{3-13}
    & &   \mcat\  & \mcat\  & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\ & \mcat\  \\
    %& &   \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\ & \dcat\  \\
    \midrule
    Ap- & Sift  & 95.2 /   96.4 /   99.6 & 93.1 /   93.1 /  94.4 & 89.5 /  90.3 /  92.7 & 89.5 /  91.1 /  92.3 & 87.1 /  87.9 /  91.5 & 89.1 /  90.7 /  91.9 & 76.6 /  79.0 /  83.9 & 54.8 /  60.5 /  67.3 & 12.5 /  16.5 /  33.5 & 1.6 /  2.4 /  8.1 & 0.0 /  0.4 /  3.6  \\
    
    GeM & D2-net   & 94.7 /  98.4 /  99.2 & 87.5 /  90.3 /  93.5 & 84.2 /  88.7 /  91.9 & 85.0 /  90.3 /  92.7 & 81.9 /  87.1 /  92.7 & 75.8 /  81.9 /  90.7 & 46.8 /  53.6 /  65.3 & 6.5 /  12.5 /  24.2 & 0.0 /  0.0 /  1.2 & 0.0 /  0.0 /  0.4 & 0.0 /  0.0 /  0.0  \\
     
     & R2D2   & 93.1 /  94.7 /  99.6 & 91.5 /  91.9 /  94.4 & 88.3 /  90.7 /  92.3 & 87.4 /  88.7 /  91.5 & 85.5 /  87.9 /  90.3 & 84.7 /  87.5 /  89.9 & 75.8 /  78.2 /  83.5 & 51.8 /  56.7 /  63.6 & 15.7 /  21.4 /  31.5 & 2.0 /  2.8 /  5.6 & 0.4 /  0.8 /  2.8 \\
     
     & SuperPoint  &  99.6 /  \textbf{100.0} /  \textbf{100.0} & 97.2 /  97.2 /  97.2 & 96.0 /  96.0 /  96.0 & 94.8 /  95.2 /  95.2 & 94.4 /  94.4 /  94.4 & 94.7 /  94.7 /  94.7 & 93.1 /  93.5 /  93.5 & 90.7 /  94.0 /  94.4 & 73.4 /  75.4 /  76.2 & 51.2 /  53.2 /  56.5 & 35.9 /  37.5 /  41.5 \\
   \midrule
    Net & Sift   &  96.4 /  97.2 /  \textbf{100.0} & 95.6 /  96.8 /  98.0 & 92.7 /  94.0 /  94.8 & 89.6 /  91.2 /  93.2 & 87.9 /  90.7 /  93.5 & 89.1 /  91.1 /  92.3 & 75.4 /  77.8 /  85.1 & 58.5 /  63.3 /  68.5 & 12.9 /  17.3 /  35.5 & 1.6 /  4.4 /  9.3 & 0.4 /  0.4 /  2.0  \\
    
    VLAD & D2-net   &  97.2 /  99.6 /  \textbf{100.0} & 89.5 /  91.9 /  96.0 & 86.7 /  89.5 /  94.0 & 85.1 /  89.1 /  94.0 & 83.1 /  88.3 /  92.7 & 78.9 /  85.8 /  90.3 & 45.2 /  58.5 /  69.4 & 10.5 /  14.5 /  28.6 & 0.0 /  0.0 /  0.8 & 0.0 /  0.0 /  0.4 & 0.0 /  0.0 /  0.0  \\
     
     & R2D2   &   91.6 /  92.8 /  99.6 & 92.7 /  94.4 /  96.4 & 88.7 /  91.1 /  92.7 & 86.3 /  89.1 /  91.1 & 85.9 /  89.1 /  90.7 & 86.3 /  89.5 /  91.5 & 76.6 /  80.6 /  87.1 & 55.1 /  59.9 /  66.0 & 14.1 /  20.2 /  33.9 & 2.0 /  2.z8 /  6.5 & 0.4 /  0.8 /  2.0 \\
     
     & SuperPoint   &  \textbf{100.0} /  \textbf{100.0} /  \textbf{100.0} & \textbf{98.8} /  \textbf{99.2} /  \textbf{99.2} & \textbf{97.2} /  \textbf{97.2} /  \textbf{97.6} & \textbf{98.4} /  \textbf{98.8} /  \textbf{98.8} & \textbf{97.6} /  \textbf{98.0} /  \textbf{98.0} & \textbf{98.0} /  \textbf{98.0} /  \textbf{98.0} & \textbf{98.0} /  \textbf{98.0} /  \textbf{98.0} & \textbf{95.2} /  \textbf{96.4} /  \textbf{96.4} & \textbf{86.7} /  \textbf{87.9} /  \textbf{88.7} & \textbf{65.1} /  \textbf{69.5} /  \textbf{72.7} & \textbf{50.0} /  \textbf{55.2} /  \textbf{58.1} \\
     

     \bottomrule
     
  \end{tabular}
  }


==> source/tables/town10_accuracies_weather.tex <==
\newcommand\mcat{T1 / T2 / T3}
\newcommand\dcat{2 / 5 / 10}
\newcommand\skiplen{0.05in}
%\tiny
  \centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{l l r r r r }
  & & \multicolumn{4}{c}{Town10}  \\
    \cmidrule{3-6}
    \vspace{-0.45cm}
    \\
    \cmidrule{3-6}
    %\midrule
         % town01
     PR & LF &  $v=$ 90 & 60 & 30 & 10 & 
    \midrule
    & &   \mcat\  & \mcat\  & \mcat\ & \mcat\  \\
    %& &   \dcat\ & \dcat\ & \dcat\ & \dcat\  \\
    \midrule
    Ap- & Sift  &  72.6 / 79.0 / 86.3 & 42.6 / 43.0 / 49.0 & 26.2 / 28.2 / 31.5 & 20.6 / 23.4 / 28.2 \\
    
     GeM & D2-net   & 63.7 / 71.0 / 81.5 & 41.5 / 44.4 / 54.8 & 30.2 / 33.1 / 40.3 & 26.1 / 29.7 / 35.3 \\
     
     & R2D2   & 72.4 / 76.8 / 82.8 & 48.6 / 51.4 / 56.3 & 33.6 / 36.8 / 40.9 & 30.2 / 31.5 / 34.3 \\
     
     & SuperPoint  & 96.0 / 96.4 / 96.4 & 89.2 / 90.0 / 90.0 & 85.9 / 86.7 / 88.7 & 85.5 / 86.7 / 87.6 \\
   \midrule
    Net- & Sift   & 77.1 / 82.3 / 88.8 & 48.8 / 51.6 / 56.5 &  30.2 / 34.3 / 37.9 & 21.8 / 23.4 / 28.2 \\
    
     VLAD & D2-net   &  62.1 / 70.6 / 82.3 & 45.6 / 50.8 / 63.3 & 35.5 / 37.1 / 44.0 & 26.2 / 31.5 / 39.1 \\
     
     & R2D2   & 77.2 / 81.2 / 86.8 & 58.1 / 59.7 / 64.1 &   40.6 / 42.2 / 46.6 & 30.6 / 34.7 / 39.5 \\
     
     & SuperPoint   & \textbf{97.6} / \textbf{97.6} / \textbf{97.6} &\textbf{97.6} / \textbf{97.6} / \textbf{97.6} & \textbf{93.1} / \textbf{94.0} / \textbf{94.0} & \textbf{89.5} / \textbf{90.7} / \textbf{91.5} \\
     
     \bottomrule
     
  \end{tabular}
  }

==> source/tables/town10_failures_illumination.tex <==
  \centering
  \begin{adjustbox}{width=\linewidth, valign=T, center}
  \begin{tabular}{l l r r r r r r r r r r r | c }
  &  &   \multicolumn{12}{c}{Town10}       \\
    \cmidrule(lr){3-14}
    %\midrule
     PR & LF &  $k=$
          % town10
     0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & CT
     \\
    %\midrule
    \midrule
    Ap- & Sift
     %town10
    &     \textbf{0.0} & 1.3 & 2.2 & 4.0 & 3.1 & 3.6 & 10.3 & 17.0 & 25.0 & 26.3 & 19.6
    %Computation time
    & 169 
    \\
     GeM & D2-net
      %town10
    &  \textbf{0.0} & 3.6 & 4.0 & 6.2 & 5.4 & 8.5 & 13.4 & 20.1 & 12.9 & 14.7 & 10.3
    %Computation time
    & 165 
     \\
     & R2D2 
      %town10
    & \textbf{0.0} & 1.8 & 4.0 & 5.8 & 5.4 & 4.9 & 9.4 & 9.8 & 20.5 & 12.9 & 13.4
    %Computation time
    & 194 
     \\
     & SuperPoint 
     %town10
     &  \textbf{0.0} & 0.9 & \textbf{0.9} & 0.4 & 1.8 & 1.3 & 1.8 & 1.8 & 3.1 & 5.8 & 12.9
     %Computation time
    & 193 
     \\
     
    \midrule
    Net- & Sift 
     % town10
    &  \textbf{0.0} & \textbf{0.0} & 1.8 & 2.2 & 0.9 & 1.8 & 6.7 & 17.9 & 34.4 & 28.1 & 21.9
     %Computation time
    & \textbf{134}  
    \\
     %
     VLAD & D2-net 
    % town10
    &  0.4 & 0.9 & 4.0 & 3.6 & 7.6 & 7.6 & 12.9 & 20.1 & 11.6 & 10.7 & 9.8
    & 139 %Computation time
    \\
     & R2D2  
     %town10
     &  \textbf{0.0} & 2.2 & 2.2 & 3.6 & 4.9 & 4.0 & 7.1 & 7.6 & 15.2 & 13.8 & 10.7
      %Computation time
    & 167 
     \\
     %town01
     & SuperPoint
     %town10
     &  \textbf{0.0} & 0.4 & \textbf{0.9} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.4} & \textbf{1.3} & \textbf{3.1} & \textbf{8.5}
   %Computation time
    & 166  
     \\
     \midrule
     \multicolumn{2}{l}{Wheel odometry} &  \multicolumn{10}{c}{9.8} & &
      \\
     \bottomrule
  \end{tabular}
  \end{adjustbox}

==> source/tables/town10_weather_failures.tex <==
\centering
    %\captionof{table}{Blalbla}
  \begin{tabular}{l l r r r r }
   & &\multicolumn{4}{c}{Town10}  \\
    \cmidrule{3-6}
    %\midrule
         % town01
    PR & LF & $v=$ 90 & 60 & 30 & 10 

     \\
    %\midrule
    \midrule
     % town01
    Ap- & Sift &  8.5 & 25.4 & 25.4 & 21.9  

    \\
     % town01
    GeM & D2-net  & 12.1 & 13.8 & 10.3 & 12.9 
     \\
      % town01
     & R2D2  & 10.3 & 12.5 & 10.3 & 10.3 
     \\
     % town01
     & SuperPoint & \textbf{0.0} & 0.4 & 1.8 & 2.2 
     \\
     
    \midrule
     % town01
    Net- & Sift  & 7.6 & 25.9 & 29.5 & 25.9 
    \\
     % town01
     VLAD & D2-net  & 12.5 & 13.4 & 10.7 & 9.4
    \\
    %town01
     & R2D2  & 9.4 & 8.0 & 7.6 & 8.5  
     \\
     %town01
     & SuperPoint  & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.9} 
     \\
     \midrule
     \multicolumn{2}{l}{Wheel odometry}  & \multicolumn{4}{c}{9.8} %& 9.8 &  &  &  
      \\
     \bottomrule
  \end{tabular}

==> source/tables/town10_weather_results.tex <==
\centering
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{ r c r r r r }
 %  & & \multicolumn{4}{c}{Town01} \\
    %\midrule
     & Visual range = & 100.0 & 10.0 & 1.0 & 0.1   \\
    \midrule
   &  Success rate & 
     100.0 & 0.0 & 0.0 & 0.0 \\
     
   Town01 & T1 / T2 / T3 &
     90.6 / 95.3 / 99.7 &
     4.3 / 10.4 / 11.7 &
     1.8 / 7.0 / 8.7 &
     4.8 / 7.0 / 10.5  \\
         \midrule

    
    % \\
 %   & &  \multicolumn{4}{c}{Town10} \\
    %     \midrule
   & Success rate & 100.0 & 10.0 & 20.0 & 40.0 \\
     
  Town10 & T1 / T2 / T3
    & 88.4 / 90.4 / 91.6 &
     51.8 / 54.2 / 57.6 &
     51.2 / 53.3 / 56.4 &
     55.5 / 57.6 / 61.2 \\

     \bottomrule
  \end{tabular}
  }


==> source/tables/weather_results_vertical.tex <==
\centering
  \resizebox{0.45\linewidth}{!}{
  \begin{tabular}{ c r r r r | r r r r }
    & \multicolumn{4}{c}{Town01} &  \multicolumn{4}{c}{Town10}\\

    \toprule
     Visual range = & 100.0 & 10.0 & 1.0 & 0.1 & 100.0 & 10.0 & 1.0 & 0.1   \\
    \midrule
     Success rate & 
     100.0 & 0.0 & 0.0 & 0.0 &
     100.0 & 10.0 & 20.0 & 40.0 \\
     
 
            T1 & 
     90.6 & 4.3 & 1.8 & 4.8 &
     88.3 & 51.8 & 51.2 & 55.5 \\
     
     T2 & 
      95.3 & 10.4 & 7.0 & 7.0 & 
     90.4 &  54.2 & 53.3 & 57.6
     \\
     
     T3 & 
     99.7 & 11.7 & 8.7 & 10.5 &
     91.6 & 57.6 & 56.4 & 61.2 
     \\

     \bottomrule
  \end{tabular}
  }


==> source/tables/weather_try.tex <==
 \centering
  \resizebox{0.6\linewidth}{!}{
  \begin{tabular}{ l r r r r }
   & \multicolumn{4}{c}{Town01}  \\
    \midrule
    %\midrule
         % town01
      &  $z=$ 0 & 2 & 4 & 5 

     \\
    %\midrule
    \midrule
     % town01
    Ap-GeM \\
    \midrule
    Sift & \textbf{0.0} & 1.3 & 5.0 & 10.4 

    \\
     % town01
      D2-net  & 0.2 & 2.8 & 29.6 & 42.2 
     \\
      % town01
      R2D2  & 0.2 & 0.7 & 7.0 & 16.2 
     \\
     % town01
      SuperPoint & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.2} 
     \\
     
    \midrule
     % town01
    NetVLAD \\
    \midrule
    Sift  & 0.2 & 1.7 & 4.0 & 9.4 
    \\
     % town01
      D2-net  & 0.3 & 2.8 & 30.1 & 40.7 
    \\
    %town01
      R2D2  & 0.2 & 0.7 & 7.8 & 16.6 
     \\
     %town01
      SuperPoint  & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & 0.5 
     \\
     \midrule
     Wheel odom &   & \hlc{18.5} &  &    
      \\
     \bottomrule
  \end{tabular}
  }

==> source/tex/navigation.tex <==
Hierarchical visual localization methods differ in
two main processing stages~\cite{sarlin_coarse_2019}: 1) prior retrieval and 2)  local feature matching.
%The hierarchical localization toolbox used in our work, HLOC~\cite{noauthor_hloc_2021}, allows testing different combinations of prior
%retrieval and local feature matching methods.

%
%
\subsection{Prior retrieval}

Prior retrieval, also known as place recognition, aims to retrieve the gallery images that are the most similar to a certain query image. This is achieved by summarising the visible scene in an image and representing it as a vector. The vectors are designed in such a way that for images representing the same scene they are similar, and for images representing different scenes they are distinctly different. The similarity of the vectors is measured by a metric such as the Euclidean or cosine distance~\cite{zaffar_vpr-bench_2021}. The earlier works on place recognition utilized a bag of visual words (BoW) approach to produce a compact representation of local descriptors such as SIFT extracted from an image~\cite{zaffar_vpr-bench_2021}. The more recent works are based on global image descriptors. In~\cite{torii_247_2015}, Torii \etal present DenseVLAD, which composes a global descriptor from local SIFT features using a Vector-of-Locally-Aggregated-Descriptors (VLAD) approach. 

The recent methods rely on convolutional neural networks (CNNs) instead of hand-engineered features. The deep learning based global image descriptors are learned end to end using a metric learning scheme leveraging a loss function such as contrastive loss, triplet loss or listwise loss~\cite{masone_survey_2021}. The deep learning methods extract dense convolutional features from an image that are, similarly to DenseVLAD, manipulated into a global descriptor by a pooling or aggregation scheme. NetVLAD~\cite{arandjelovic_netvlad_2018} is a seminal work in the field. In their paper, Arandjelovic \etal propose adding a learnable VLAD layer on top of a CNN feature extractor. A similar approach was adopted by Radenovic \etal, who proposed replacing the VLAD layer with a learnable generalized mean (GeM) layer~\cite{radenovic_fine-tuning_2019}. Revaud \etal extended upon this in their work on Ap-GeM~\cite{revaud_learning_2019} by replacing the contrastive loss with a novel listwise average precision (Ap) loss function. In~\cite{hausler_patch-netvlad_2021}, Hausler \etal divide an image to patches for which they extract global descriptors to improve over the performance of the original NetVLAD model. In their paper~\cite{vedaldi_unifying_2020} (DELG), Cao \etal propose a model which jointly learns local and global feature extractors using a multi-task learning scheme. Finally, in~\cite{leyva-vallina_generalized_2021} Leyva-Vallina \etal utilize a novel generalized contrastive loss to perform learning on non-binary ground truth labels.

%
%
\subsection{Local feature matching}

%\begin{figure}[b]
%  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%   \includegraphics[width=0.3\linewidth]{source/figures/Tavaraa(2).png}
%   \caption{Benchmark implementation overview}
%   \label{fig:system_overview}
%\end{figure}

Once the images that contain parts of the scene that overlap with those visible in a query image have been retrieved, the exact geometric relationship between the query and gallery images can be estimated by utilizing local correspondences. The local correspondences are commonly estimated using a multi-stage approach~\cite{ma_image_2021}. First, interest points which are likely to provide stable descriptors are detected. Then, a descriptor representing the image pixels around the interest point is extracted. A good descriptor is robust to changes in viewpoint and appearance. Finally, the descriptors from different images are matched in order to find image-to-image correspondences. As with place recognition methods, in earlier works the correspondences were found by matching hand-engineered feature descriptors like SIFT across the images. In recent years, deep learning has gained popularity in this area of research too. 

SuperPoint~\cite{detone_superpoint_2018} is a CNN feature point detector and descriptor that is trained end-to-end in a self-supervised way. The network has distinct branches for both feature detection and description, and these are trained using separate loss functions. In their work on D2-net~\cite{dusmanu_d2-net_2019}, Dusmanu \etal utilize a similar learning-based approach. However, instead of first detecting and then describing interest points, they learn detection and description within a single branch of the network. R2D2~\cite{revaud_r2d2_2019} by Revaud \etal aims at learning feature descriptors that are both reliable and repeatable. The network has three output branches: the descriptors, a repeatability map and a reliability map. These are learned in a self-supervised fashion using a list-wise loss formulation. DISK~\cite{tyszkiewicz_disk_2020} is inspired by reinforcement learning methods, and utilizes policy gradient to match descriptors between images. LoFTR \cite{sun_loftr_2021} utilizes a transformer network to extract image correspondences in a detector-free manner. The positional encoding and attention mechanism of the transformer enable LoFTR to find matches even in low-texture areas, a task at which detect-and-describe schemes often struggle.

%\vspace{-\medskipamount}

\paragraph{Matcher.}
To determine image correspondences, the extracted descriptors have to be matched. At its simplest form, this can be done by a nearest neighbour (NN) search. The performance of NN matching can be improved by using heuristics such as the ratio test~\cite{ma_image_2021}. The ratio test considers as correct matches only those descriptor pairs where the distance of a descriptor to its first NN is significantly smaller than its distance to the second NN. The ratio between these two distances is used as the threshold. For the rest of the paper, we shall denote nearest neighbour matcher with ratio test as NN-ratio. Learning based methods present an alternative to NN matchers. SuperGlue~\cite{sarlin_superglue_2020} uses a graph neural network to match SuperPoint descriptors by solving an optimal transport problem. The descriptor correspondences acquired using the matchers can be filtered for outliers using geometric constraints with variants of RANSAC. For a comprehensive survey on local descriptors and descriptor matching, we refer the reader to~\cite{ma_image_2021}. 


==> source/tex/results_cvpr.tex <==
%
% Experiment 1
\subsection{Illumination change}

\begin{table*}[h]
\input{source/tables/town01_successrates}
%\begin{subtable}{0.573\linewidth}
%    \input{source/tables/town01_successrates}
%    \caption{The navigation success rates over 5 repeated runs of the same route. }
%  \label{tab:town01_success_rates}
%  \end{subtable}
%  \begin{subtable}{0.407\linewidth}
%    \input{source/tables/town10_successrates}
%    \caption{The navigation success rates over 5 repeated runs of the same route. }
%  \label{tab:town10_success_rates}
%  \end{subtable}
  \caption{The navigation success rates over 5 repeated runs of the same route. I$^\dagger$ shows the rate for 10 runs with artificial street illumination. }
  \label{tab:success_rates}
\end{table*}

\begin{table*}
    \input{source/tables/town01_accuracies_short}
    \caption{The visual localization recall rates over 5 test runs. The accuracy thresholds used are T1 ($\le$ 0.25m, $\le$2$^\circ$),
    T2 ($\le$0.50m,$\le$5$^\circ$) and
    T3 ($\le$5.00m, $\le$10$^\circ$).  I$^\dagger$ denotes artificial street illumination results. Full table for all $k$ values in the supplementary material.
    %using different combinations of visual localization methods. To save space, the accuracies are shown here for even values of $k$. The full table for all $k$-values can be found in the appendix.
    % 
    }
    \label{tab:town01_accuracies}
\end{table*}

%\begin{figure}[!b]
%  \centering
%  
%  \begin{subfigure}{0.48\linewidth}
%    \includegraphics[width=0.95\linewidth]{source/figures/failureplace_map01.png}
%    \caption{Onboard camera photo of a building.}
%    \label{fig:failureplace_town01}
%  \end{subfigure}
%  \begin{subfigure}{0.48\linewidth}
%    \includegraphics[width=0.95\linewidth]{source/figures/failure_causer_map01.png}
%    \caption{Another building along the route.}
%    \label{fig:failurecauser_town01}
%  \end{subfigure}
%  \par\medskip
%  
%    \begin{subfigure}{0.5\linewidth}
%    \includegraphics[width=0.95\linewidth]{source/figures/failureplace_overview.png}
%    \caption{Overview of the place of failure}
%    \label{fig:failureplace-overview_town01}
%  \end{subfigure}
% 
%  \caption{A spot along the route in Town01 where visual localization methods often fail. Two similar buildings along the route often cause localization algorithms two confuse the locations of the two, leading to the vehicle driving off route. Brightness of the images has been adjusted for better viewing. \hl{REMOVE TO SAVE SPACE?}}
%  \label{fig:failureim_town01}
%\end{figure}


Table~\ref{tab:success_rates} shows the success rates of visual navigation under different illumination conditions. The success rates are computed over five repeated runs. Variance between the runs come from the fact that computation times of visual localization vary and thus poses are retrieved and control signals generated for different locations in different runs. All visual localization pipelines perform well when the
query run corresponds to the gallery data ($k=0$). However,
the success rates quickly drop when the scene dims toward night
time.
%All of the localization method combinations succeed in navigating the test route autonomously when the test illumination correspond to those of the gallery set. When the amount of illumination is decreased, differences rapidly arise between the localization combinations.
While the both prior retrieval methods, Ap-GeM and NetVLAD,
perform well with all descriptors and matchers, the combination of NetVLAD, SuperPoint and SuperGlue is
clearly superior to others. In Town01 this combination achieves 100\% navigation success rate at $k=7$, corresponding to illumination parameter values less than $1/100$th those of the gallery conditions. One possible explanation for the large margin could be the pretraining conducted with synthetic data that is a part of the SuperPoint training process~\cite{detone_superpoint_2018}.

There is no great difference in success rates between the two test maps, Town01 and Town10.
%For most of the methods there is only minor variation between the different environments.
This indicates that the validity of the results
%is not limited to a single experimental design, but
can be generalised to a wider range of maps with the same illumination conditions.

Table~\ref{tab:town01_accuracies} includes the visual localization accuracies for the same runs. When interpreting the results the reader should note that for test cases where the success rate is below 100\%, the accuracies are not fully comparable as the numbers are
for images before the car crashes. This, in some cases, can cause the impression that the recall rates rise as the amount of illumination is decreased.
%For a scenario execution in which the autonomous vehicle crashes before reaching the end of the route, the accuracy is reported from localizations up to the point of crash. This means that for failed executions the localization accuracy is evaluated for just a sub-sequence of the full test route.
The relationship between the success rates and localization accuracy is interesting. Many of the methods achieve success rates of 0\% even if the localization accuracy is moderately good. The lowest accuracy at which a method combination achieves 100\% success rate for an illumination condition is 93.1\% @ $0.25m$, $2\deg$ for NetVLAD+SuperPoint+SuperGlue at $k=6$ in Town10.
This high rates have been reported only rarely %for a few methods
for real data~\cite{sattler_benchmarking_2018}.
%This is an accuracy so high that only few of the methods tested in
%or other benchmarks reach such values with real data.

%\vspace{-2\medskipamount}

\paragraph{Discussion.}
It is noteworthy that even though a visual localization
pipeline can correctly recall over 80\% of images
within 0.25 meters and 2$^\circ$ accuracy the
autonomous navigation fails and the car crashes even on
empty streets. This result suggests that visual localization methods are already sufficiently accurate and localization failures should be solved in other layers of the navigation stack.

There are certain inconsistencies in the success rates.
For example, 
%More interesting patterns can be observed between the different $k$-values within the same environment. Performance of
Ap-GeM combined with SuperPoint in Town10 fails
almost always for
%is an example. The success rate stays close to 0\% for 
$k$-values between 3 and 6, but for $k=7$ the rate again
raises.
%to is a rise in success rate, which reaches 60\%.
A similar pattern is observed for NetVLAD combined with SuperPoint in Town01 at $k$-values 6 and 7. % combine with below paragraph
%
There are two reasons for this behavior. The first
is
the pure pursuit controller that is able to suppress the
effect of erroneous estimates. Infrequent localization
errors that appear far away from the current location yield to
slowly changing steering angle that keep the vehicle
near the correct track to the next waypoint.
The second reason is perceptual aliasing in the environment, \eg repeated textures or visually similar objects appearing along different parts of the route, that lead to such situations and differently depending on the illumination intensity. Example images of these cases are added to our supplementary material.

%\vspace{-2\medskipamount}
\paragraph{Artificial illumination}

Tables~\ref{tab:success_rates} and~\ref{tab:town01_accuracies} also show the results from the artificial illumination experiment. The autonomous vehicle manages to complete the route more often in Town10. The reason for this is the scene structure: in Town01, the camera of the vehicle is aimed at a poorly lit area for part of the route. On that segment, only the curb close to the vehicle is well visible. This makes it difficult for the localization algorithm to find feature matches. The overall success rate of navigation is still over 50\%, which is a demonstration of the robustness of the visual localization method to severe gallery-to-query appearance change.

% COMMENTED TO MAKE SPACE
%One reason for this is that the controller utilized in this study utilizes the pose estimates from the visual localization algorithm, without any motion model or filtering approach. As such, the autonomous vehicle is very fragile to even temporary errors in pose estimation, and a single failed estimate can cause the vehicle to drive off the road. Perceptual aliasing in the environment, \eg repeated textures or visually similar objects appearing along different parts of the route, can easily lead to such situations. Combined with gallery-to-query appearance change, this can result in highly unstable behavior of the visual localization. 

% COMMENTED TO MAKE SPACE
%An example can be seen in Table~\ref{tab:success_rates} at $k$ values 6 and 7 for NetVLAD+SuperPoint in Town01. At $k=6$, the specific combination of perceptual aliasing and illumination change leads to a localization failure that causes the vehicle to crash on each of the 5 navigation attempts. At $k=7$, the combination doesn't lead to such a localization failure, and the success rate rises to 100\% from 0\% of the previous illumination condition even though the amount of light is lower. A similar pattern can be observed for Ap-GeM+SuperPoint in Town10. The success rate stays close to 0\% for $k$-values between 3 and 6. However, for value 7 there is a rise in success rate, which reaches 60\%. The failures for $k$-values 3-6 are caused by a repetitive texture. At $k=7$, the combination of the illumination and the texture is such that the agent manages to navigate past the perceptually aliased building.
%%Figure~\ref{fig:failureim_town01} shows typical a typical cause of failure in Town01. 

%It should be noted that our
%%In some cases the properties of the
%pure pursuit controller is able to suppress the
%effect of
%%smoothen the effect of highly
%erroneus estimates. If the vehicle believes it is very far from its next navigation goal, the trajectory to the goal is along the arc of a large circle, which often means that the car will continue on an almost straight course until the next estimate arrives with a more accurate pose. This opens an important research question: In which layer of the navigation stack (Figure~\ref{fig:system_overview}) the errors should be deal with? Our benchmark provides a framework to
%systematically study these important research questions.

% PERHAPS WHERE OUR SYSTEM CAN BE USED to StudY:
%Since it's unlikely that visual localization would achieve accuracies in the range of $> 95\%$ in real environments, for any practical systems it should probably be accompanied by complementary localization methods. One approach could be fusing the pose estimate from visual localization with data from IMU and wheel odometry. Visual pose estimates could be used to correct the drift of these relative positioning systems, and they in turn would prevent a single erroneus visual pose estimate from leading the vehicle off track. This could be implemented in the simulator benchmark too, providing a future topic of research.

%\vspace{-1\medskipamount}

\subsection{Weather change}

Here we present the results from the weather change experiments. Table~\ref{tab:weather_accuracies} shows the success and recall rates for NetVLAD + SuperPoint + SuperGlue. With no fog, the success rates are at 100\% which is in line with the results at $k=6$ from Table~\ref{tab:success_rates}. When the amount of fog is increased, the success and recall rates quickly drop. Still, on some of the test runs the vehicle is able to complete the full route even under very foggy conditions. A pattern similar to the one observed in the illumination experiments is visible here as well: the success rate first drops, then grows a bit. Here too, the explanation can be found from perceptual aliasing.

\begin{table}[h]
    \input{source/tables/town10_weather_results}
    %\input{source/tables/weather_results_vertical}
    \caption{The navigation success and visual localization recall rates over 10 runs at different visual ranges for NetVLAD + SuperPoint + SuperGlue. Thresholds T1-T3 are the same. %as in the previous experiments.
    %used are $\le$ 0.25m and  $\le$2$^\circ$ (T1),
    %$\le$0.50m and $\le$5$^\circ$ (T2) and
    %$\le$5.00m and $\le$10$^\circ$ (T3). 
    }
    \label{tab:weather_accuracies}
\end{table}

